Factor Fields: A Unified Framework for Neural Fields and Beyond

We present Factor Fields, a novel framework for modeling and representing signals. Factor Fields decomposes a signal into a product of factors, each represented by a classical or neural field representation which operates on transformed input coordinates. This decomposition results in a unified framework that accommodates several recent signal representations including NeRF, Plenoxels, EG3D, Instant-NGP, and TensoRF. Additionally, our framework allows for the creation of powerful new signal representations, such as the "Dictionary Field" (DiF) which is a second contribution of this paper. Our experiments show that DiF leads to improvements in approximation quality, compactness, and training time when compared to previous fast reconstruction methods. Experimentally, our representation achieves better image approximation quality on 2D image regression tasks, higher geometric quality when reconstructing 3D signed distance fields, and higher compactness for radiance field reconstruction tasks. Furthermore, DiF enables generalization to unseen images/3D scenes by sharing bases across signals during training which greatly benefits use cases such as image regression from sparse observations and few-shot radiance field reconstruction.

==> figs/framework.tex <==
  \begin{overpic}[width=\linewidth]{figs/teaser.pdf}

    \put(8.3,31.5) { \small Point $\bx$ }

    \put(19,33) { \small  $\bgamma_1$ }
    \put(19,28.0) { \small $\bgamma_i$ }
    \put(19,25) { \small $\bgamma_N$ }

    \put(43.4,26) { \large  $($}
    \put(48.9,26) { \large  $\circ$}
    \put(50.7,26.) { \large $\cdots$ }
    \put(53.9,26) { \large  $\circ$}
    \put(59.3,26) { \large  $)$}

    
    % \put(24.5,37) { \large $\Transform(\bx)$ }
    \put(26,33) { \small Sinusoidal$(\bx$) }
    \put(26,31) { \small Triangular$(\bx)$ }
    \put(26,29) { \small Sawtooth$( \bx)$ }
    \put(26,27) { \small Hashing$( \bx)$ }
    \put(26,25) { \small Orthogonal-1D$(\bx)$}
    \put(26,23) { \small Orthogonal-2D$(\bx)$ }
    \put(26,21) { \small Polynomial$(\bx)$ }
    \put(26,19.5) { \small $\cdots$ }

    % \put(22.7,14.5) { \small $\bx_\Phi$ }
    % \put(34.4,14.5) { \small $\bx_\Psi$ }
    
    \put(9,17) { \small Coordinates }
    \put(21,17) { \small Coordinate Transformation }
    
    \put(42.9,17) { \small $\bff_1(\bgamma_1(\bx))$ }
    \put(52.4,17) { \small $\bff_N(\bgamma_N(\bx))$ }
    
    \put(74.3,17) { \small Projection Function }

    \put(1.2,11) { \footnotesize Field Representations $\bff_i$}
    \put(2.3,0.9) { \footnotesize Polynomial }
    \put(16.0,0.9) { \footnotesize MLPs }
    \put(26.9,0.9) { \footnotesize $3$D Grids }
    \put(39.1,0.9) { \footnotesize $2$D Maps }
    \put(50.3,0.9) { \footnotesize $1$D Vectors }
    \put(76.5,0.9) { \footnotesize Outputs }
  \end{overpic}

==> figs/imagesSet.tex <==
  \begin{overpic}[width=0.98\linewidth]{figs/images/imageSet.jpg}
    \put(6, -2) { \small \textbf{(1)} \footnotesize Image set 256$\times3\times$1024$\times$1024 (size); \footnotesize \SI{43.88}{\mega\nothing} (params); \footnotesize 28.66 dB (average PSNR)}
    \put(75, 24) { \small \textbf{(2)} coefficients visualization}

    \put(69.2, 0.8) { \small $L_1$}
    \put(77, 0.8) { \small $L_2$}
    \put(84, 0.8) { \small $L_3$}
    \put(89.3, 0.8) { \small $L_4$}
    \put(92.9, 0.8) { \small $L_5$}
    \put(96.6, 0.8) { \small $L_6$}
    \put(77.5, -2) { \small \textbf{(3)} basis visualization}
  \end{overpic}


==> secs/appx.tex <==

\begin{table*}[htpb]
    \vspace{2em}
    \centering
    \begin{tabular}{l|c|cccccccc}
    \hline
    Methods & Avg. & {\it Chair} & {\it Drums} & {\it Ficus} & {\it Hotdog} & {\it Lego} & {\it Materials} & {\it Mic} & {\it Ship} \\
    \hline\hline
    \multicolumn{9}{@{}l}{\rule{0pt}{3ex}\bf PSNR$\uparrow$} \\
    \hline
    SRN~\cite{sitzmann2019scene} & 22.26 & 26.96 & 17.18 & 20.73 & 26.81 & 20.85 & 18.09 & 26.85 & 20.60 \\
    NeRF~\cite{mildenhall2020nerf} & 31.01 & 33.00 & 25.01 & 30.13 & 36.18 & 32.54 & 29.62 & 32.91 & 28.65 \\
    NSVF~\cite{liu2020neural} & 31.75 & 33.19 & 25.18 & 31.23 & 37.14 & 32.29 & 32.68 & 34.27 & 27.93 \\
    SNeRG~\cite{hedman2021baking} & 30.38 & 33.24 & 24.57 & 29.32 & 34.33 & 33.82 & 27.21 & 32.60 & 27.97 \\
    PlenOctrees~\cite{yu2021plenoctrees} & 31.71 & 34.66 & 25.31 & 30.79 & 36.79 & 32.95 & 29.76 & 33.97 & 29.42 \\
    Plenoxels~\cite{yu2021plenoxels} & 31.71 & 33.98 & 25.35 & 31.83 & 36.43 & 34.10 & 29.14 & 33.26 & 29.62 \\
    DVGO~\cite{sun2021direct} & 31.95 & 34.09 & 25.44 & 32.78 & 36.74 & 34.64 & 29.57 & 33.20 & 29.13 \\
    TensoRF & 33.14 & 35.76 & 26.01 & 33.99 & 37.41 & 36.46 & 30.12 & 34.61 & 30.77 \\
    instant-NGP & 33.14 & 35.76 & 26.01 & 33.99 & 37.41 & 36.46 & 30.12 & 34.61 & 30.77 \\
    
    \hline
    NeuBasis (ours) & 33.14 & 35.76 & 26.01 & 33.99 & 37.41 & 36.46 & 30.12 & 34.61 & 30.77 \\

    \hline
    \end{tabular}
    \caption{PSNR results on each scene from the {\bf Synthetic-NeRF}~\cite{mildenhall2020nerf} dataset. %Ours $^\dag$ refers to our tensorf representation with direct optimization (i.e., without network) while ours are trained with a small MLP network.
    }
    \label{tab:supp_breakdown_nerf}
    \vspace{2em}
\end{table*}

\begin{table*}[htpb]
    \vspace{2em}
    \centering
    \begin{tabular}{l|c|cccccccc}
    \hline
    Methods & Avg. & {\it Chair} & {\it Drums} & {\it Ficus} & {\it Hotdog} & {\it Lego} & {\it Materials} & {\it Mic} & {\it Ship} \\
    \hline\hline
    % \multicolumn{9}{@{}l}{\rule{0pt}{3ex}\bf PSNR$\uparrow$} \\
    % \hline
    % SRN~\cite{sitzmann2019scene} & 22.26 & 26.96 & 17.18 & 20.73 & 26.81 & 20.85 & 18.09 & 26.85 & 20.60 \\
    % NeRF~\cite{mildenhall2020nerf} & 31.01 & 33.00 & 25.01 & 30.13 & 36.18 & 32.54 & 29.62 & 32.91 & 28.65 \\
    % NSVF~\cite{liu2020neural} & 31.75 & 33.19 & 25.18 & 31.23 & 37.14 & 32.29 & 32.68 & 34.27 & 27.93 \\
    % SNeRG~\cite{hedman2021baking} & 30.38 & 33.24 & 24.57 & 29.32 & 34.33 & 33.82 & 27.21 & 32.60 & 27.97 \\
    % PlenOctrees~\cite{yu2021plenoctrees} & 31.71 & 34.66 & 25.31 & 30.79 & 36.79 & 32.95 & 29.76 & 33.97 & 29.42 \\
    % Plenoxels~\cite{yu2021plenoxels} & 31.71 & 33.98 & 25.35 & 31.83 & 36.43 & 34.10 & 29.14 & 33.26 & 29.62 \\
    % DVGO~\cite{sun2021direct} & 31.95 & 34.09 & 25.44 & 32.78 & 36.74 & 34.64 & 29.57 & 33.20 & 29.13 \\

    % \hline
    % Ours-CP-384  & 31.56 & 33.60 & 25.17 & 30.72 & 36.24 & 34.05 & 30.10 & 33.77 & 28.84 \\
    % Ours-VM-192-SH  & 32.00 & 34.68 & 25.37 & 32.30 & 36.30 & 35.42 & 29.30 & 33.21 & 29.46 \\
    % Ours-VM-48  & 32.39 & 34.68 & 25.58 & 33.37 & 36.81 & 35.51 & 29.45 & 33.59 & 30.12 \\
    % Ours-VM-192-15k & 32.52 & 34.95 & 25.63 & 33.46 & 36.85 & 35.78 & 29.78 & 33.69 & 30.04\\
    % Ours-VM-192-30k & 33.14 & 35.76 & 26.01 & 33.99 & 37.41 & 36.46 & 30.12 & 34.61 & 30.77 \\
    % \hline
    
    % \hline
    
    % \hline    

    \multicolumn{9}{@{}l}{\rule{0pt}{3ex}\bf SSIM$\uparrow$} \\
    \hline
    SRN~\cite{sitzmann2019scene} & 0.846 & 0.910 & 0.766 & 0.849 & 0.923 & 0.809 & 0.808 & 0.947 & 0.757 \\
    NeRF~\cite{mildenhall2020nerf} & 0.947 & 0.967 & 0.925 & 0.964 & 0.974 & 0.961 & 0.949 & 0.980 & 0.856 \\
    NSVF~\cite{liu2020neural} & 0.953 & 0.968 & 0.931 & 0.973 & 0.980 & 0.960 & 0.973 & 0.987 & 0.854 \\
    SNeRG~\cite{hedman2021baking} & 0.950 & 0.975 & 0.929 & 0.967 & 0.971 & 0.973 & 0.938 & 0.982 & 0.865 \\
    PlenOctrees~\cite{yu2021plenoctrees} & 0.958 & 0.981 & 0.933 & 0.970 & \gold{0.982} & 0.971 & \gold{0.955} & 0.987 & 0.884 \\
    Plenoxels~\cite{yu2021plenoxels} & 0.958 & 0.977 & 0.933 & 0.976 & 0.980 & 0.976 & 0.949 & 0.985 & 0.890 \\
    DVGO~\cite{sun2021direct} & 0.957 & 0.977 & 0.930 & 0.978 & 0.980 & 0.976 & 0.951 & 0.983 & 0.879 \\
    TensoRF & 0.963 & 0.985 & 0.937 & 0.982 & 0.982 & 0.983 & 0.952 & 0.988 & 0.895 \\
    instant-NGP & 0.963 & 0.985 & 0.937 & 0.982 & 0.982 & 0.983 & 0.952 & 0.988 & 0.895 \\
    \hline
    
    NeuBasis (ours) & 0.963 & 0.985 & 0.937 & 0.982 & 0.982 & 0.983 & 0.952 & 0.988 & 0.895 \\
    
    \hline
    
    \hline    


    \multicolumn{9}{@{}l}{\rule{0pt}{3ex}\bf LPIPS$_{VGG}\downarrow$ } \\
    \hline
    SRN~\cite{sitzmann2019scene} & 0.170 & 0.106 & 0.267 & 0.149 & 0.100 & 0.200 & 0.174 & 0.063 & 0.299 \\
    NeRF~\cite{mildenhall2020nerf} & 0.081 & 0.046 & 0.091 & 0.044 & 0.121 & 0.050 & 0.063 & 0.028 & 0.206 \\

    PlenOctrees~\cite{yu2021plenoctrees}  & 0.053 & 0.022 & 0.076 & 0.038 & \gold{0.032} & 0.034 & 0.059 & 0.017 & 0.144 \\
    Plenoxels~\cite{yu2021plenoxels}  & 0.049 & 0.031 & \gold{0.067} & 0.026 & 0.037 & 0.028 & \gold{0.057} &\gold{0.015} & \gold{0.134} \\
    DVGO~\cite{sun2021direct} & 0.053 & 0.027 & 0.077 & 0.024 & 0.034 & 0.028 & 0.058 & 0.017 & 0.161 \\
    TensoRF & 0.047 & 0.022 & 0.073 & 0.022 & 0.032 & 0.018 & 0.058 & 0.015 & 0.138 \\

    %s
    \hline
    \multicolumn{9}{@{}l}{\rule{0pt}{3ex}\bf LPIPS$_{Alex}\downarrow$} \\
    NSVF~\cite{liu2020neural}  & 0.047 & 0.043 & 0.069 & 0.017 & 0.025 & 0.029 & 0.021 & 0.010 & 0.162 \\
    DVGO~\cite{sun2021direct}  & 0.035 & 0.016 & 0.061 & 0.015 & 0.017 & 0.014 & \gold{0.026} & 0.014 & 0.118 \\
    
    
     \hline
    Ours-CP-384        & 0.041 & 0.022 & 0.069 & 0.024 & 0.024 & 0.014 & 0.031 & 0.018 & 0.130 \\
    Ours-VM-192-SH     & 0.058 & 0.031 & 0.082 & 0.028 & 0.048 & 0.024 & 0.069 & 0.022 & 0.160  \\
    Ours-VM-48         & 0.032 & 0.014 & 0.059 & 0.015 & 0.017 & 0.009 & 0.036 & 0.012 & 0.098 \\
    Ours-VM-192-15k        & 0.032 & 0.013 & 0.056 & 0.014 & 0.017 & 0.009 & 0.029 & 0.013 & 0.101 \\
    Ours-VM-192-30k        & \gold{0.027} & \gold{0.010} & \gold{0.051} & \gold{0.012} & \gold{0.013} & \gold{0.007} & \gold{0.026} & \gold{0.009} & \gold{0.085} \\
    \hline

    \end{tabular}
    \caption{Quantitative results on each scene from the {\bf Synthetic-NeRF}~\cite{mildenhall2020nerf} dataset. %Ours $^\dag$ refers to our tensorf representation with direct optimization (i.e., without network) while ours are trained with a small MLP network.
    }
    \label{tab:supp_breakdown_nerf}
    \vspace{2em}
\end{table*}

\newpage
\begin{figure*}[htbp]
    \includegraphics[width=\linewidth]{figs/res_nerf.pdf}
    \caption{Our rendering results on {\bf Synthetic-NeRF} dataset. From top to bottom: Ship, Hotdog, Lego, Mic, Chair, Drums, Materials, Ficus.}
    \label{fig:synthetic_nerf}
\end{figure*}

==> secs/related.tex <==
\section{Related Work}
\boldstartspace{Neural Representation.}

\boldstartspace{Sparse Coding and Dictionary Learning.}

